Learning to Predict Distributions over Weight Updates for Test-Time Adaptation

Hypernetworks have recently shown success in dynamically adapting the parameters of Large Language Models (LLMs) at runtime based on signals such as task descriptions or additional demostrations. Here we ask: how much adaptation signal can be obtained using only the input query to an LLM?. To answer this, we study query-conditioned Hypernetworks for LoRA estimation. Further, we introduce distributional Hypernetworks, able to produce not only point estimates of parameter adaptors, but also a distribution over possible LoRAs. For this we propose a simple end-to-end loss using a differentiable Monte Carlo approximation and explore multiple distribution parametrizations including regression and convex combination variants. Results show that even using the mean of the learned distribution can outperform deterministic hypernetworks. Crucially, the learned distribution enables a different form of test-time scaling: instead of spending additional compute only by sampling more token sequences from a fixed model, we sample weight updates, yielding multiple adapted models for the same query. Performance improves as more weight samples are considered and remains stronger than corresponding token-sampling adaptation baselines. Finally, we find that generated updates can transfer across queries, suggesting that the hypernetwork learns reusable structure in how the model should adapt. Together, these results show that query-conditioned distributions over weight updates can support both adaptation and test-time scaling.

==> scripts/sync-remote <==
#!/usr/bin/env bash

set -euo pipefail

resolve_with_codex=false

usage() {
  printf '%s\n' \
    'Usage: scripts/sync-remote [--resolve-with-codex]' \
    '' \
    'Pulls the current branch with rebase, then pushes it.' \
    'Tracked changes must be committed first; untracked files are ignored.' \
    '' \
    'Options:' \
    '  --resolve-with-codex  Ask Codex CLI to resolve pull conflicts.' \
    '  -h, --help            Show this help.'
}

while (($#)); do
  case "$1" in
    --resolve-with-codex)
      resolve_with_codex=true
      ;;
    -h|--help)
      usage
      exit 0
      ;;
    *)
      printf 'Unknown option: %s\n\n' "$1" >&2
      usage >&2
      exit 2
      ;;
  esac
  shift
done

repo_root=$(git rev-parse --show-toplevel)
cd "$repo_root"

if [[ -n $(git status --porcelain --untracked-files=no) ]]; then
  printf '%s\n' 'Refusing to sync: commit or discard tracked changes first.' >&2
  git status --short --untracked-files=no >&2
  exit 1
fi

if ! git pull --rebase; then
  if [[ -z $(git diff --name-only --diff-filter=U) ]] &&
     [[ ! -d "$(git rev-parse --git-path rebase-merge)" ]] &&
     [[ ! -d "$(git rev-parse --git-path rebase-apply)" ]]; then
    printf '%s\n' 'Pull failed without merge conflicts; not pushing.' >&2
    exit 1
  fi

  if [[ $resolve_with_codex != true ]]; then
    printf '%s\n' \
      'Pull stopped with conflicts.' \
      'Resolve them manually, or rerun with --resolve-with-codex.' >&2
    exit 1
  fi

  if ! command -v codex >/dev/null 2>&1; then
    printf '%s\n' 'Cannot resolve conflicts: Codex CLI is not installed.' >&2
    exit 1
  fi

  codex exec \
    --approve-for-me \
    --sandbox workspace-write \
    --cd "$repo_root" \
    --ephemeral \
    'Resolve only the current Git pull/rebase conflicts. Preserve the intent of both local and remote changes. Inspect the relevant surrounding code, remove every conflict marker, run focused validation when practical, and continue the rebase if one is active. Do not create an unrelated commit and do not push. Finish only when Git reports no unmerged paths; otherwise explain the blocker and exit unsuccessfully.'

  if [[ -n $(git diff --name-only --diff-filter=U) ]]; then
    printf '%s\n' 'Codex returned with unresolved conflicts; not pushing.' >&2
    exit 1
  fi

  if [[ -d "$(git rev-parse --git-path rebase-merge)" || -d "$(git rev-parse --git-path rebase-apply)" ]]; then
    printf '%s\n' 'A rebase is still active; not pushing.' >&2
    exit 1
  fi
fi

git push

